Learning to Generate 3D Shapes with Generative Cellular Automata

We present a probabilistic 3D generative model, named Generative Cellular Automata, which is able to produce diverse and high quality shapes. We formulate the shape generation process as sampling from the transition kernel of a Markov chain, where the sampling chain eventually evolves to the full shape of the learned distribution. The transition kernel employs the local update rules of cellular automata, effectively reducing the search space in a high-resolution 3D grid space by exploiting the connectivity and sparsity of 3D shapes. Our progressive generation only focuses on the sparse set of occupied voxels and their neighborhood, thus enabling the utilization of an expressive sparse convolutional network. We propose an effective training scheme to obtain the local homogeneous rule of generative cellular automata with sequences that are slightly different from the sampling chain but converge to the full shapes in the training data. Extensive experiments on probabilistic shape completion and shape generation demonstrate that our method achieves competitive performance against recent methods.

==> experiments.tex <==
% !TeX root = ./main.tex
\section{Experiments}



\begin{table}[t]
    \begin{minipage}[t]{0.47\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{figures/generation_results.png}
        \captionof{figure}{Generation Results}
        \label{generation_results}
    \end{minipage}
    \hspace{0.03\linewidth}
    \begin{minipage}[t]{0.5\linewidth}
        \vspace{0pt}
        \centering
        \includegraphics[width=\linewidth]{figures/completion_results.png}
        \captionof{figure}{Probabilistic Completion Qualitative Comparison}
        \label{completion_results}
    \end{minipage}
    
\end{table}


We demonstrate the ability of GCA to generate high-fidelity shapes in two tasks: shape generation (Sec.~\ref{sec:shape_generation}) and probabilistic shape completion (Sec.~\ref{sec:shape_completion}).
% State-of-the-art works on both tasks generate a fixed number of point cloud whereas ours uses grid structure.
State-of-the-art works on both tasks generate shapes using point cloud whereas ours uses grid structure.
For comparison, we extracted high-resolution points from the CAD model and map them into $64^3$ voxel grid.
Individual shapes in the dataset are centered and uniformly scaled to fit within the cube $[-1,1]^3$.
The ablation study (Sec.~\ref{sec:ablation}) examines how the sparse representation and local transition can successfully learn to generate  fine resolution shapes with continuous geometry.
Details regarding the training model architecture and experimental settings are stated in the appendix~\ref{experimental_details}


\if 0
In this section, we evaluate the proposed GCA in the task of shape generation (\ref{sec:shape_generation}) and probabilistic shape completion(\ref{sec:shape_completion}).
Then we present an ablation study examining design choices of our approach.
Implementation details are shown in the appendix.

To our knowledge, no other recent works on each tasks have been performed with voxel representation.
Thus we compare our method against recent state-of-the art methods that employ the point cloud representation.
For all experiments, we extract points from the CAD model, and normalize all point clouds by centering the bounding boxes to the origin and scale them by a constant so that all points range within the cube $[-1, 1]^3$.
Then we voxelize the point cloud to match the resolution of $64^3$.
\fi

\subsection{Shape Generation} \label{sec:shape_generation}

\input{generation_table}


\textbf{Dataset and implementation details.} 
We test the performance of shape generation using the ShapeNet (\cite{chang2015shapenet}) dataset, focusing on the categories with the most number of shapes, \textit{airplane, car,} and \textit{chair} as presented in \cite{yang2019pointflow}.
We use the same experimental setup as \cite{cai2020shapegf}, and sample 2,048 points from the occupied cells of the generate shape for fair comparison.
We use neighborhood size $r = 2$ with $L_1$ metric, $T = 100$ inferences, and infusion speed $w = 0.005$.

The quantitative results of shape generation are reported in Table \ref{table:generation_comparison}.
We compare the performance of our approach against recent point cloud based method: r-GAN (\cite{achlioptas2017latent_pc}), GCN-GAN (\cite{valsesia2019gcngan}), Tree-GAN (\cite{shu2019treegan}), Pointflow (\cite{yang2019pointflow}), and ShapeGF (\cite{cai2020shapegf}).
We evaluate our model on three metrics, minimal matching distance (MMD), coverage (COV), and 1-nearest-neighbor-accuracy (1-NNA)
as defined in the appendix~\ref{evaluation_metrics}.

Our method outperforms all of compared approaches in terms of MMD, which indicates that the approach can generate high-fidelity shapes.
% We believe that the sparse convolutional network can make high-resolution observation of neighborhood context than point-based representation. 
Our approach also achieves the state-of-the art results on COV of \textit{car} and \textit{chair}, implying that the method is able to generate diverse results, and comparable results in terms of 1-NNA (comparing distribution of generated shapes and test set).
Note we are using a homogeneous transition kernel confined within the local neighborhood of occupied cells, but can still achieve noticeable performance to generate the rich distribution of shape.
We demonstrate selected examples of our shape generation results in Figure~\ref{generation_results}.
More qualitative results are in the appendix~\ref{sec:qualitative_appendix}.


\if 0
\textbf{Dataset.} 
Our experiments focus mainly on ShapeNet (\cite{chang2015shapenet}), which contains 3D CAD models from various categories.
Following the work of \cite{cai2020shapegf}, we train our approach in airplane, car, and chair categories.

\textbf{Compared Methods.}
We quantitatively compare performance of our approach against recent point cloud based method: r-GAN (\cite{achlioptas2017latent_pc}), GCN-GAN (\cite{valsesia2019gcngan}), Tree-GAN (\cite{shu2019treegan}), Pointflow (\cite{yang2019pointflow}), ShapeGF (\cite{cai2020shapegf}).
We use the same experiment setup as ShapeGF, where we sample 2,048 points from the generated set for fair comparison.


\textbf{Evaluation Metrics.}
Following prior works (\cite{achlioptas2017latent_pc, yang2019pointflow}),  we evaluate our model on 3 metrics, minimal matching distance (MMD), coverage (COV), and 1-nearest-neighbor-accuracy (1-NNA).
MMD and COV, proposed by \cite{achlioptas2017latent_pc}, measures the fidelity and diversity of the generated set.
\cite{lopez2015revisiting} propose to use nearest neighbor to compare the distribution of generated and test point cloud set.
The detailed description regarding evaluation metrics are found in the appendix~\ref{evaluation_metrics}.



\textbf{Results.}
The quantitative results are reported in Table \ref{table:generation_comparison}.
For all generation results, we use neighborhood of size 2 with $L_1$ metric, and $T = 100$ inferences.
We outperform all other methods by a significant margin in MMD, which shows that our method generates high-fidelity shapes.
Our approach also achieves state-of-the art results on COV of car and chair, implying that the method is able to generate diverse results.
\fi

\subsection{Probabilistic Shape Completion} \label{sec:shape_completion}

\input{completion_table}

\textbf{Dataset and implementation details.}
The probabilistic shape completion is tested with PartNet (\cite{mo2019partnet}) and PartNet-Scan (\cite{wu2020multimodal}) dataset, where objects in ShapeNet are annotated with instance-level parts.
For each instance, we identify the input partial object by randomly choosing parts from the complete shape, and generate a diverse set of complete shape.
PartNet-Scan dataset simulates the real-world situation where partial scans suffer from part-level incompleteness by randomly selecting parts from the PartNet and virtually scanning the remaining parts.
We validate our approach on \textit{chair, lamp}, and \textit{table} categories following \cite{wu2020multimodal}.
For \textit{chair} and \textit{table} dataset, we use neighborhood size $r=2$ with $L_1$ metric, $T = 50$ inferences, and infusion speed $w = 0.01$.
On the \textit{lamp} dataset, we use neighborhood radius $r=3$, $T=70$ with infusion speed $w = 0.005$, since the shapes of lamp tend to be disconnected.
We further discuss the connectivity in Section~\ref{connectivity}.
Following the work of \cite{wu2020multimodal}, we generate 10 completion results for each partial shape in the test set.


We compare the performance of probabilistic shape completion of GCN against cGAN (\cite{wu2020multimodal}) and its variations (cGAN-im-l2z and cGAN-im-pc2z), which is the only shape completion method that is able to generate diverse shapes to the best of our knowledge.\footnote{We would like to acknowledge that when training, cGAN only requires the partial set and complete shape set, without any explicit pairing between each of the instances in the set.
However, we report cGAN as baseline to our method, since this is the only approach announced in probabilistic shape completion.
cGAN-im-l2z and cGAN-im-pc2z are variants of cGAN that implicitly model the multi-modality for probabilistic shape completion. }
The qualitative results  in Figure~\ref{completion_results} and the appendix (Figure~\ref{completion_results_appendix}) clearly show that our high-resolution completion exhibit clear geometric details compared to the state-of-the-art.
Our superior performance is further verified in the quantitative results reported in Table \ref{table:completion_comparison}, where three distances are given between the generated set and the test set: minimal matching distance (MMD), total mutual distance (TMD), and unidirectional Hausdorff distance (UHD).
The detailed description regarding the evaluation metrics are found in the appendix~\ref{evaluation_metrics}.
We outperform all other methods by large margin in MMD and TMD and we achieve comparable or the best results in UHD.
The results indicates that we can generate high fidelity (MMD) yet diverse (TMD) shapes while being loyal to the given partial geometry (UHD).
Especially we observed extremely diverse shapes in from \textit{lamp} datasets, which is the dataset with the most diverse structure.
We believe that the translation invariance of our model is directly related to capture the diverse structure in the data.
We include further discussion about the diversity in \textit{lamp} dataset in the appendix~\ref{lamp_diversity}.


%We outperform all other methods by a large margin in MMD and UHD, demonstrating that we can generate high fidelity shapes (MMD) while being loyal to the given partial geometry (UHD).
%TMD indicates the diversity of the generated set, and we observed extremely diverse shapes in from \textit{lamp} datasets, which is diverse in structure in the given dataset to start with.
%We believe that the translation invariance of our model is directly related to capture the diverse structure in the data.
%We discuss further regarding the diversity in \textit{lamp} dataset in the appendix~\ref{lamp_diversity}.


\if 0
\textbf{Dataset.}
For probabilistic completion, we employ the PartNet dataset (\cite{mo2019partnet}) where objects in ShapeNet are annotated by instance-level part.
For each instance in the dataset, we identify partial object by randomly choosing parts from the complete shape.
To simulate the real-world situation where partial scans suffer from part-level incompleteness, we also conduct experiments on PartNet-Scan, as in \cite{wu2020multimodal}.
The fractional data of PartNet-Scan are created by randomly selecting parts from the PartNet and virtually scanning the remaining parts.
We validate our approach on chair, lamp, table categories.

\textbf{Evaluation Metrics.}
Following the work of \cite{wu2020multimodal}, we generate 10 completion results for each partial shape in the test set.
Then, we compare 3 distances, minimal matching distance (MMD), total mutual distance (TMD), unidirectional Hausdorff distance (UHD), between the generated set and the test set.
MMD and TMD measures the quality and the diversity of the generated set.
UHD measures the completion fidelity to the input partial. 
Details regarding metrics are reported in the appendix (\ref{evaluation_metrics}).

\textbf{Compared Methods.} 
To our knowledge, cGAN (\cite{wu2020multimodal}) is the only shape completion method that is able to generate diverse shapes.
We would like to acknowledge that when training, cGAN only requires the partial set and complete shape set, without any explicit pairing between each of the instances in the set.
However, we report cGAN as baseline to our method, since this is the only approach announced in probabilistic shape completion.
We compare our method against cGAN and it's variants cGAN-im-l2z and cGAN-im-pc2z, which both implicitly model the multimodality when completing the partials. 


\input{completion_table}

\textbf{Results.} 
The quantitative results of probabilistic shape completion are reported in Table \ref{table:completion_comparison}.
For chair and table dataset, we used neighborhood of size 2 with $L_1$ metric, and $T = 50$ inferences.
On the lamp dataset, we used neighborhood of size 5, since the shapes of lamp tend to be disconnected.
We further discuss the connectivity in section~\ref{connectivity}.
We outperform all other methods by a large margin MMD and UHD, generating high fidelity shapes while being loyal to the input partial.
We saw extremly diverse shapes in from lamp datasets.
We believe that one of the reason was due to the translation invariant nature of our model.
We discuss further about regarding the diversity in lamp dataset in the appendix.
\fi


\subsection{Ablation Study}\label{sec:ablation}


\begin{table}[t]
    \begin{minipage}[t]{0.5\linewidth}
        \vspace{0pt}
        \scalebox{0.9}{\input{figures/searchspace_all.pgf}}
        \captionof{figure}{Search space visualization.
        Solid / dashed lines visualize the percentage of occupied / searched voxels during 100 time steps of generation with respect to the whole grid space.}
        \label{search_space}
    \end{minipage}
    \hspace{0.5cm}
     \begin{minipage}[t]{0.45\linewidth}
        \vspace{5pt}
        \centering
        \includegraphics[width=\linewidth]{figures/lamp_disconnected.png}
        \captionof{figure}{
        Completing disconnected shapes with $r = 3$, $L_1$ metric  neighborhood, where diameter of lamp is over 30.
        Top, front, side view of generation process is shown.
        GCA is able to generate body of the lamp that is disconnected with the given partial lamp head.
        % The stochasticity of our model generates a temporary bridge.
        }
        \label{lamp_disconnected}
    \end{minipage}
    \vspace{-1em}
\end{table}


%\begin{figure}
%    \begin{center}
%        \input{figures/searchspace_all.pgf}
%    \end{center}
%    \captionof{figure}{Search space visualization. Solid / dashed lines visualize the percentage of occupied / searched voxels during 100 time steps of generation with respect to the whole grid space.}
%    \label{search_space}
%\end{figure}


\subsubsection{Search Space Analysis}
\label{sec:ab_searchspace}
In this section we analyze the effectiveness of the sparse representation of our approach.
One major hurdle of voxel-based representation to handle 3D shape is the required memory. 
However, we could make a high-resolution predictions by only handling the occupied voxels and their neighborhood. 
% The percentage of occupied voxel depends on the actual shape of the data.
We empirically observe in Figure~\ref{search_space} that the occupied voxels take approximately 2\% of the total volume (solid lines), and their neighborhood is around 2-8\% (dashed lines).
Therefore, the size of search space  for our algorithm requires reasonable amount of memory  during the entire shape generation process and still make detailed prediction in fine resolution.
After certain amount of time steps, the size of the search space stops increasing implying that our method is able to converge and maintain the generated shape.




\subsubsection{Effects of Neighborhood Size}
In this section, we further investigate the effect of radius $r$ of the neighborhood size. 
We experiment by changing the neighborhood radius $r$ on probabilistic completion with lamp dataset.
When $r = 1$, nearly 10\% of the infusion chain data failed to meet the ending criterion with time step $T = 100$, unable to learn the full shape of training data $x$.
% This lead to an increase of 30\% MMD and 6\% UHD, not being able to generate high fidelity shapes.
We believe that small neighborhood size failed to model disconnected shapes even with large time steps.
On the other hand, when $r = 10$, this led to an highly unstable training generating some noise-like blurry output or results highly unrelated to the input partial.
We believe that due to enormous search space, neighborhood size increasing cubic to $r$, sampling few bad steps led to an irreversible states that was either far from states observed during training or completely new state compared to the previous state.


\subsubsection{Connectivity} \label{connectivity}

In this section, we clarify the meaning of connectivity used in our approach.
One might misunderstand that our model can generate only cells that are directly connected to the previous state, meaning that GCA cannot generate shapes divided into multiple parts.
However, our approach is more flexible and capable of generating parts within the neighborhood distance $r$.
% The size of the search space $r$ is directly related to the capability of learning to generate parts that is $r$ apart.
Also, we should take into account that $r$ is the distance of cells between immediate steps and it is possible to  learn the sequence of states that generates a temporary \textit{bridge} to reach disconnected parts after a few steps.
Figure~\ref{lamp_disconnected} shows an observed sequence of sampling chain that generates a temporary bridge from the body to generate the head of lamp located further than the neighborhood size and removes the bridge afterwards.



==> gca.tex <==
% !TeX root = ./main.tex
\section{Generative Cellular Automata}

\begin{figure}	
	\includegraphics[width=\linewidth]{teaser}
	\caption[Sampling Chain of GCA shape generation.] {
		Sampling chain of shape generation.
		Each row shows a sample starting from a single voxel at the left most column.
		Our model progressively evolves to a shape from the learned distribution.
		Each column shows samples after applying 5 transition operations from the previous one, and the right most column is the final generated sample after total of 100 transition operations. 
	}
\end{figure}

%\subsection{Notations and Problem Setup}
\input{gca_problem_setup}
\input{gca_local_update_rules}
% \input{gca_inference}
\input{gca_training}


==> gca_inference.tex <==
% !TeX root = ./main.tex
\subsection{Sampling Procedure}

We define the generative model $p$ to follow the sampling procedure starting with initial state $s^0 = x$, and repeatedly applying the stochastic transition kernel $p(s^{t + 1} | s^t)$, creating Markov chain $s^0 \rightarrow s^1 \rightarrow ...\rightarrow s^{T - 1}$ named \textit{sampling chain}.
$s^{T - 1}$ is considered as the final generated sample and the joint probability is given by $p(s^{T - 1}) = \Sigma_{s^{0:T - 2}} p(s^0) \prod_{0 < t < {T - 1}} p(s^{t + 1} | s^t)$.
Each transition is designed to deform the current state to the learned shape following the local update rules of CA.
\begin{figure}
	\includegraphics[width=\linewidth]{main_figure_no_arrow}
	\caption[Overview] {
		Overview our model.
		The top shows a probabilistic shape completion sampling chain of a chair starting from the partial input.
		Bottom figures show an illustrative figure of our method.
		Starting from a sampled chain $s^t$, we apply sparseCNN to obtain the neighborhood occupancy probability of next state.
		Then we aggregate the probabilities cellwise averaging and sample the next state from it.
	}
\end{figure}

==> gca_local_update_rules.tex <==
% !TeX root = ./main.tex
\subsection{Local Update Rule}
We provide a detailed explanation of modeling the local update rules of CA efficiently utilizing sparse CNN.
The sparse CNN maps the input state of $M$ cells $s^t = \{c_1, \cdots, c_M\}$ into $N$-dimension vectors $\mathcal{P} = \{\mathbf{p}_1, \cdots, \mathbf{p}_M \}$
 \footnote{
	The features associated to coordinates are set to 1, where using a fully convolutional neural network makes the model translation invariant.
},
where $N$ is the size of the neighborhood and $\mathbf{p}_k \in [0, 1]^N$ is the occupancy probability for the cells of $N(\{c_k\})$.
The elements of $\mathbf{p}_k$ are $N$ cells that belong to $N(\{c_k\})$, sorted by the relative position with respect to $c_k$, and contain the probability for the cells being occupied following the Bernoulli distribution.
For example, the first and second elements of output could represent the probabilities of the top-left and top of the occupied cell in 2 dimensional grid.
We ignore the cells that do not belong to neighborhood of current state 	$N(s^t)$ assuming that they have the probability of 0 occupancy.
This way, we maintain the sparsity of intermediate states.

The probability distribution of the neighborhood of $\mathbf{p}_k$ overlaps when the occupied cells are close to each other.
We average the multiple estimated probabilities for each cells in $N(s^t)$, thus estimating the probability of all the coordinates in $N(s^t)$.
Overview of the sampling procedure and the local update rule is depicted in Figure~\ref{overview}.

\begin{figure}
	\includegraphics[width=\linewidth]{main_figure_no_arrow}
	\caption[Overview] {
		Overview our model.
		The top shows a probabilistic shape completion sampling chain of a chair starting from the partial input.
		Bottom figures show an illustrative figure of our method.
		Starting from a sampled chain $s^t$, we apply sparse CNN to obtain the neighborhood occupancy probability of next state.
		Then we aggregate the probabilities by cellwise averaging and sample the next state from it.
	}
	\label{overview}
\end{figure}





==> gca_problem_setup.tex <==
% !TeX root = ./main.tex
\subsection{Problem Setup}

Let $\mathds{Z}^d$ be a $d$-dimensional uniform grid space, where $d=3$ for 3D voxel space.
Each cell in the grid space can have values of occupied (1) or empty (0).
\footnote{Note that we are using surface-based representation to exploit the sparsity and mark 1 when the surface lies, instead of a conventional volumetric occupancy grid}.
Since the allowed values for each grid is binary, each shape can be represented as an ordered set of occupied coordinates of occupied grid cells $s \subset \mathds{Z}^d$, which we define as a state.
Union ($\cup$), intersection ($\cap$) and subset ($\subset$) between states are defined as regular sets, given that states are defined as sets of coordinates.

We define the neighborhood state $N(s) = \bigcup_{c \in s }\{c' \in \mathds{Z}^d |\;  d(c, c') \leq r\}$ of state $s$, where $d$ is a distance function between two coordinates in $\mathds{Z}^d$, and $r$ is a fixed constant.
For example, the neighborhood of a state with a single cell in 2 dimension with $r = 1$ and $L_{\infty}$ metric is a square surrounding the coordinate.
% \footnote{This is referred as Moore neighborhood in cellular automata.}

\if 0
We will denote pair $(x, y)$ as samples from the dataset $\mathcal{D}$, where $y$ is the shape that we wish to generate and $x$ is the initial shape.
The initial shape depends on the task we aim to solve.
For the task of probabilistic shape completion, $x$ and $y$ are partial and complete shape.
For shape generation, we set the initial state $x = \{c\}$ to be the most simple solution that we can think of, a single cell $c$.
\fi 

We are interested in a sequence of continuous state variables $s^{0:T}$ that is drawn from the following Markov chain:
\begin{equation}
	s^0  \sim p^0	\quad s^{t + 1} \sim p_\theta(s^{t + 1} | s^t), \quad 0 \leq t < T
\end{equation}
where $p_\theta$ is the homogeneous transition kernel parameterized by $\theta$ and $p^0$ is some initial distribution.
We will denote the Markov chain $s^0 \rightarrow s^1 \rightarrow ...\rightarrow s^{T}$ with transition kernel $p$, named \textit{sampling chain}, and the marginal probability of the final generated sample is given by 
\begin{equation}
p(s^{T}) = \sum_{s^{0:T - 1}} p^0(s^0) \prod_{0 < t < T} p(s^{t + 1} | s^t).
\end{equation}
Given empirical data distribution $q^*$ associated to data set $\mathcal{D}$ containing 3D shapes $x \in \mathcal{D}$, our objective is to learn the parameters $\theta$ of transition kernel $p$, such that 
\begin{enumerate}
	\item distribution of final generated sample $p(s^T)$ is close to data distribution $q^*$ 
	\item each transition kernel follows the local update rules of CA, reducing the search space of sparse and connected voxel space, i.e. $s^{t + 1} \subset N(s^t)$
\end{enumerate}

\if 0
to follow the sampling procedure starting with initial state $s^0 = x$, and repeatedly applying the stochastic transition kernel $p(s^{t + 1} | s^t)$, creating Markov chain $s^0 \rightarrow s^1 \rightarrow ...\rightarrow s^{T - 1}$ named \textit{sampling chain}.
$s^{T - 1}$ is considered as the final generated sample and the joint probability is given by $p(s^{T - 1}) = \Sigma_{s^{0:T - 2}} p(s^0) \prod_{0 < t < {T - 1}} p(s^{t + 1} | s^t)$.
Each transition is designed to deform the current state to the learned shape following the local update rules of CA.
\fi

\if 0
We are interested in a sequence of random state variables $s^{0:T}$, that is drawn from the following Markov chain:
\begin{equation*}
	s^0 \sim \pi^0 \quad s^{t + 1} \sim p(s^{t + 1} | s^t)
\end{equation*}
where $p$ is a homogeneous transition kernel and $\pi^0$ is the initial distribution for 

Our objective is to learn a transition operator $p(s^{t + 1} | s^t)$, such that repeated application produces sample from the data manifold and follow the local update rules of the CA, reducing the search space, i.e. $s^{t + 1} \subset N(s^t)$. 
\fi
